An Inverse Modeling Constrained Multi-Objective Evolutionary Algorithm Based on Decomposition

This paper introduces the inverse modeling constrained multi-objective evolutionary algorithm based on decomposition (IM-C-MOEA/D) for addressing constrained real-world optimization problems. Our research builds upon the advancements made in evolutionary computing-based inverse modeling, and it strategically bridges the gaps in applying inverse models based on decomposition to problem domains with constraints. The proposed approach is experimentally evaluated on diverse real-world problems (RWMOP1-35), showing superior performance to state-of-the-art constrained multi-objective evolutionary algorithms (CMOEAs). The experimental results highlight the robustness of the algorithm and its applicability in real-world constrained optimization scenarios.

==> Tables/IMC.tex <==
\begin{table*}[ht]
\scalefont{0.9}
\centering
\label{tab:imc}
\caption{Means and standard deviation of the Hypervolume metric on RWMOP1-35. Best performances are Highlighted. Settings for the population size ($N$), the number of objectives ($m$), decision variables ($d$), the maximum of fitness evaluation ($FE$), and quantity of inequality ($ng$) and equality ($nh$) constraints for each test problem.}
\begin{tabular}{@{}ccccccccccc@{}}
\hline
Problem & $N$ & $m$ & $d$ & $ng$ & $nh$ & $FE$  & IM-C-MOEA                                           & \multicolumn{1}{c|}{IM-MOEA}                                   & IM-C-MOEA/D                                         & IM-MOEA/D                                 \\ \hline
\multicolumn{11}{c}{Mechanical Design Problems}                                                                                                                                                                                                                          \\
RWMOP1  & 80  & 2   & 4   & 2    & 2    & 20000 & \hl{4.6051e-1 (3.13e-2) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{5.8560e-1 (7.39e-3) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP2  & 80  & 2   & 5   & 5    & 0    & 20000 & \hl{3.6766e-1 (7.79e-3) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{3.3757e-1 (3.56e-2) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP3  & 80  & 2   & 3   & 3    & 0    & 20000 & \hl{8.6356e-1 (6.18e-3) +}         & \multicolumn{1}{c|}{1.9427e-1 (2.74e-1)}                       & \hl{7.1513e-1 (4.62e-2) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP4  & 80  & 2   & 4   & 4    & 0    & 20000 & \hl{7.8057e-1 (2.14e-2) +}         & \multicolumn{1}{c|}{2.9166e-1 (2.62e-1)}                       & \hl{5.0765e-1 (9.09e-2) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP5  & 80  & 2   & 4   & 4    & 0    & 20000 & \hl{4.2608e-1 (7.55e-4) +}         & \multicolumn{1}{c|}{2.6687e-1 (1.78e-2)}                       & \hl{4.2795e-1 (8.56e-4) +}         & 2.3416e-1 (6.83e-3)                       \\
RWMOP6  & 80  & 2   & 7   & 11   & 0    & 20000 & \hl{2.7533e-1 (2.31e-4) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{2.7468e-1 (3.49e-4) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP7  & 80  & 2   & 4   & 1    & 0    & 20000 & \hl{4.7110e-1 (1.89e-3) +}         & \multicolumn{1}{c|}{4.6305e-1 (2.97e-3)}                       & \hl{4.7906e-1 (2.08e-3) +}         & 4.7157e-1 (5.36e-3)                       \\
RWMOP8  & 105 & 3   & 7   & 9    & 0    & 26250 & \hl{2.3507e-2 (3.31e-4) +}         & \multicolumn{1}{c|}{2.0817e-2 (8.62e-4)}                       & \hl{2.3871e-2 (4.29e-4) +}         & 1.6289e-2 (1.46e-3)                       \\
RWMOP9  & 80  & 2   & 4   & 0    & 0    & 20000 & \hl{3.6739e-1 (8.50e-3) $\approx$} & \multicolumn{1}{c|}{3.6587e-1 (7.52e-3)}                       & \hl{4.0321e-1 (2.05e-3) +}         & 3.3149e-1 (1.72e-2)                       \\
RWMOP10 & 80  & 2   & 2   & 2    & 0    & 20000 & 8.3546e-1 (4.69e-3) $\approx$                       & \multicolumn{1}{c|}{\hl{8.3677e-1 (3.71e-3)}} & \hl{8.4480e-1 (5.81e-4) +}         & 8.3696e-1 (2.18e-3)                       \\
RWMOP11 & 212 & 5   & 3   & 7    & 0    & 53000 & \hl{8.4717e-2 (2.04e-3) +}         & \multicolumn{1}{c|}{7.1942e-2 (3.29e-3)}                       & \hl{9.0599e-2 (1.47e-3) +}         & 7.5898e-2 (2.86e-3)                       \\
RWMOP12 & 80  & 2   & 4   & 1    & 0    & 20000 & \hl{4.9200e-1 (1.73e-2) +}         & \multicolumn{1}{c|}{2.0577e-1 (1.20e-1)}                       & \hl{4.0147e-1 (5.92e-2) +}         & 2.1557e-4 (1.18e-3)                       \\
RWMOP13 & 105 & 3   & 7   & 11   & 0    & 26250 & \hl{8.6440e-2 (2.76e-4) +}         & \multicolumn{1}{c|}{1.1527e-3 (6.31e-3)}                       & \hl{8.7439e-2 (1.99e-4) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP14 & 80  & 2   & 5   & 8    & 0    & 20000 & \hl{5.3033e-1 (1.75e-2) +}         & \multicolumn{1}{c|}{1.3503e-1 (1.15e-1)}                       & \hl{4.9617e-1 (3.39e-2) +}         & 4.4961e-2 (3.41e-2)                       \\
RWMOP15 & 80  & 2   & 3   & 8    & 0    & 20000 & \hl{4.9915e-1 (6.04e-3) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{2.8940e-1 (7.85e-2) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP16 & 80  & 2   & 2   & 2    & 0    & 20000 & \hl{7.1653e-1 (1.01e-2) +}         & \multicolumn{1}{c|}{6.1425e-1 (7.77e-2)}                       & \hl{5.6697e-1 (7.51e-2) +}         & 1.1608e-1 (3.79e-3)                       \\
RWMOP17 & 105 & 3   & 6   & 9    & 0    & 26250 & \hl{1.9777e-1 (2.98e-2) +}         & \multicolumn{1}{c|}{1.6645e-2 (6.33e-2)}                       & \hl{1.9138e-1 (4.20e-2) +}         & 1.9777e-2 (5.91e-2)                       \\
RWMOP18 & 80  & 2   & 3   & 3    & 0    & 20000 & \hl{3.8177e-2 (3.28e-4) +}         & \multicolumn{1}{c|}{3.6332e-2 (8.30e-4)}                       & \hl{4.0302e-2 (8.05e-5) +}                               & 3.9935e-2 (2.12e-4) \\
RWMOP19 & 105 & 3   & 10  & 10   & 0    & 26250 & \hl{3.2244e-1 (6.73e-3) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{3.2377e-1 (4.52e-3) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP20 & 80  & 2   & 4   & 7    & 0    & 20000 & 0.0000e+0 (0.00e+0) $\approx$                       & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\
RWMOP21 & 80  & 2   & 6   & 4    & 0    & 20000 & \hl{3.1130e-2 (2.39e-4) +}         & \multicolumn{1}{c|}{3.1048e-2 (1.61e-4)}                       & \hl{3.1405e-2 (6.63e-5) +}         & 3.0760e-2 (7.36e-6)                       \\
\multicolumn{11}{c}{Chemical Engineering Problems}                                                                                                                                                                                                                       \\
RWMOP22 & 80  & 2   & 9   & 2    & 4    & 20000 & 0.0000e+0 (0.00e+0) $\approx$                       & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\
RWMOP23 & 80  & 2   & 6   & 1    & 4    & 20000 & \hl{1.1034e-1 (1.59e-1) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\
RWMOP24 & 105 & 3   & 9   & 0    & 6    & 26250 & 0.0000e+0 (0.00e+0) $\approx$                       & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\
\multicolumn{11}{c}{Process, Design, and Synthesis Problems}                                                                                                                                                                                                              \\
RWMOP25 & 80  & 2   & 2   & 2    & 0    & 20000 & \hl{2.1984e-1 (2.41e-3) +}         & \multicolumn{1}{c|}{1.7608e-1 (1.07e-1)}                       & \hl{2.3916e-1 (1.36e-3) +}         & 2.3282e-1 (1.85e-5)                       \\
RWMOP26 & 80  & 2   & 3   & 1    & 1    & 20000 & \hl{1.6593e-1 (2.45e-2) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{1.7561e-1 (1.94e-2) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP27 & 80  & 2   & 3   & 3    & 0    & 20000 & \hl{1.9524e+2 (2.44e+2) +}         & \multicolumn{1}{c|}{1.0780e-1 (3.31e-1)}                       & \hl{1.4589e+5 (4.60e+5) +}         & 5.2170e+2 (2.30e+3)                       \\
RWMOP28 & 80  & 2   & 7   & 4    & 4    & 20000 & 0.0000e+0 (0.00e+0) $\approx$                       & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\
RWMOP29 & 80  & 2   & 7   & 9    & 0    & 20000 & \hl{6.9427e-1 (1.18e-1) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{7.5814e-1 (3.19e-2) +}         & 0.0000e+0 (0.00e+0)                       \\
\multicolumn{11}{c}{Power Electronics Problems}                                                                                                                                                                                                                          \\
RWMOP30 & 80  & 2   & 25  & 24   & 0    & 80000 & \hl{3.4240e-2 (1.07e-1) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{1.0268e-1 (2.36e-1) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP31 & 80  & 2   & 25  & 24   & 0    & 80000 & \hl{1.5029e-2 (5.78e-2) $\approx$} & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{2.0911e-2 (1.15e-1) $\approx$} & 0.0000e+0 (0.00e+0)                       \\
RWMOP32 & 80  & 2   & 25  & 24   & 0    & 80000 & \hl{5.5420e-2 (1.53e-1) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & \hl{9.9896e-2 (2.59e-1) +}         & 0.0000e+0 (0.00e+0)                       \\
RWMOP33 & 80  & 2   & 30  & 29   & 0    & 80000 & 0.0000e+0 (0.00e+0) $\approx$                       & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\
RWMOP34 & 80  & 2   & 30  & 29   & 0    & 80000 & 0.0000e+0 (0.00e+0) $\approx$                       & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\
RWMOP35 & 80  & 2   & 30  & 29   & 0    & 80000 & \hl{2.7882e-2 (7.35e-2) +}         & \multicolumn{1}{c|}{0.0000e+0 (0.00e+0)}                       & 0.0000e+0 (0.00e+0) $\approx$                       & 0.0000e+0 (0.00e+0)                       \\ \hline
\multicolumn{7}{c}{+/-/$\approx$}               & 26/0/9                                              & \multicolumn{1}{c|}{}                                          & 26/0/9                                              &                                           \\ \hline
\end{tabular}
\end{table*}
